Event-Based De-Snowing for Autonomous Driving

Adverse weather conditions, particularly heavy snowfall, pose significant challenges to both human drivers and autonomous vehicles. Traditional image-based de-snowing methods often introduce hallucination artifacts as they rely solely on spatial information, while video-based approaches require high frame rates and suffer from alignment artifacts at lower frame rates. Camera parameters, such as exposure time, also influence the appearance of snowflakes, making the problem difficult to solve and heavily dependent on network generalization. In this paper, we propose to address the challenge of desnowing by using event cameras, which offer compressed visual information with submillisecond latency, making them ideal for de-snowing images, even in the presence of ego-motion. Our method leverages the fact that snowflake occlusions appear with a very distinctive streak signature in the spatio-temporal representation of event data. We design an attention-based module that focuses on events along these streaks to determine when a background point was occluded and use this information to recover its original intensity. We benchmark our method on DSEC-Snow, a new dataset created using a green-screen technique that overlays pre-recorded snowfall data onto the existing DSEC driving dataset, resulting in precise ground truth and synchronized image and event streams. Our approach outperforms state-of-the-art de-snowing methods by 3 dB in PSNR for image reconstruction. Moreover, we show that off-the-shelf computer vision algorithms can be applied to our reconstructions for tasks such as depth estimation and optical flow, achieving a $20\%$ performance improvement over other de-snowing methods. Our work represents a crucial step towards enhancing the reliability and safety of vision systems in challenging winter conditions, paving the way for more robust, all-weather-capable applications.

==> sections/biography.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{floats/photo/manasi.jpg}}]{Manasi Muglikar} %
received her PhD from the University of Zurich (UZH), under the supervision of Prof. Davide Scaramuzza, with a focus on low-latency computational imaging using event cameras.
She obtained her B.E in Electrical and Electronics from BITS Pilani, India in 2016 and M.S in Electrical and Computer Engineering from Carnegie Mellon University (CMU) in 2017.
Her work has received awards such as the Best Systems Paper Award at Robotics: Science and Systems (RSS) 2020 and UZH Forschungskredit Grant 2023.
\end{IEEEbiography}
\vskip -2.6\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{floats/photo/nico.jpg}}]{Nico Messikommer} holds an M.Sc. in Robotics, Systems, and Control from ETH Zürich, Switzerland, which he obtained in 2019 following his B.Sc. in Mechanical Engineering in 2017. 
He received his Ph.D. in Computer Science from the University of Zurich under the supervision of Prof. Davide Scaramuzza.
His research centers on the intersection of computer vision and robotics, exploring topics such as unsupervised domain adaptation, event cameras, and reinforcement learning. 
His contributions were recognized by the nomination as an Award Candidate at the 2023 Conference on Computer Vision and Pattern Recognition (CVPR).
\end{IEEEbiography}
\vskip -2.6\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{floats/photo/marco_cannici.jpg}}]{Marco Cannici} 
 received the M.Sc. degree in computer science and engineering, and Ph.D. degree in information technology from Politecnico di Milano, Milano, Italy, in 2018 and 2022, respectively.,From 2022 to 2025, he was a Postdoctoral Researcher with the Robotics and Perception Group, University of Zurich, Zurich, Switzerland, under the supervision of Prof. Davide Scaramuzza. He is currently a Researcher with the Smart Eyewear Lab, a joint platform initiative between EssilorLuxottica and the Politecnico di Milano, where he develops event-based perception and sensing systems for smart glasses. His research focuses on event-based vision and perception for autonomous systems, spanning from visual odometry and monocular obstacle avoidance to high-speed and low-latency perception and 3-D reconstruction in challenging conditions.

\end{IEEEbiography}
\vskip -2.6\baselineskip plus -1fil


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{floats/photo/davide.jpg}}]{Davide Scaramuzza} %
is a Professor of Robotics and Perception at the University of Zurich. He did his Ph.D. at ETH Zurich, a postdoc at the University of Pennsylvania, and was a visiting professor at Stanford University. His research focuses on autonomous, agile microdrone navigation using standard and event-based cameras. He pioneered autonomous, vision-based navigation of drones, which inspired the navigation algorithm of the NASA Mars helicopter and many drone companies. He contributed significantly to visual-inertial state estimation, vision-based agile navigation of microdrones, and low-latency, robust perception with event cameras, which were transferred to many products, from drones to automobiles, cameras, AR/VR headsets, and mobile devices. In 2022, his team demonstrated that an AI-controlled, vision-based drone could outperform the world champions of drone racing, a result that was published in Nature. He is a consultant for the United Nations on disaster response and disarmament. He has won many awards, including an IEEE Technical Field Award, the IEEE Robotics and Automation Society Early Career Award, a European Research Council Consolidator Grant, a Google Research Award, two NASA TechBrief Awards, and many paper awards. In 2015, he co-founded Zurich-Eye, today Meta Zurich, which developed the world-leading virtual-reality headset Meta Quest. In 2020, he co-founded SUIND, which builds autonomous drones for precision agriculture. Many aspects of his research have been featured in the media, such as The New York Times, The Economist, and Forbes.
\end{IEEEbiography}
\vskip -2.6\baselineskip plus -1fil
